Motif-based Convolutional Neural Network on Graphs

This paper introduces a generalization of Convolutional Neural Networks (CNNs) to graphs with irregular linkage structures, especially heterogeneous graphs with typed nodes and schemas. We propose a novel spatial convolution operation to model the key properties of local connectivity and translation invariance, using high-order connection patterns or motifs. We develop a novel deep architecture Motif-CNN that employs an attention model to combine the features extracted from multiple patterns, thus effectively capturing high-order structural and feature information. Our experiments on semi-supervised node classification on real-world social networks and multiple representative heterogeneous graph datasets indicate significant gains of 6-21% over existing graph CNNs and other state-of-the-art techniques.

==> motif.tex <==
Conventionally, a motif (or metagraph) has been defined as a pattern of edges among different node types~\cite{science,metagraph}. To model 
%Since such a definition does not model the
locality specific to a node type, we additionally demarcate the structural roles of the context node and auxiliary nodes. 
%we propose a novel definition of motifs that describes the receptive field around a given node type) and demarcates the structural roles of various context nodes. 
We define a graph motif $M$ as a subgraph composed of a designated \textit{target} node $t_M$, \textit{context} node $c_M$ and a relevant subset of \textit{auxiliary} nodes $B_M$, whose roles are determined by their type and structural symmetry relative to $t_M$.
Formally,\\
%, we describe a motif as below: \\
\textbf{Definition 1:} \textit{A motif $M$ with target $t_M$, context $c_M$ and auxiliary nodes $B_M$ is defined as $M = (V_M, E_M, B_M, t_M, c_M)$ with node type mapping $l_M: V_M \mapsto \mathcal{L}$ where $V_M$ is a set of nodes with $t_M, c_M \in V_M$  and $B_M \subseteq V_M - \{t_M,c_M\}$, $E_M$ is a set of edges and $ \forall x \in V_M, l_M(x) \in \mathcal{L}$.}

We define an instance $S_u$ of motif $M$ with target $u$ in $G$ as a subgraph induced by $M$ with $u$ as the target node. Formally, \\
%The formal definition of an instance is given by: \\
\textbf{Definition 2:} \textit{An instance $S_u = (V_S, E_S) $ of motif $M$ with target node $u$ on $G$ is a subgraph of $G$ where $V_S \subseteq V$ and $E_S \subseteq E$, such that there exists a bijection  $ \psi_S : V_S \mapsto V_M $ satisfying (i) $u \in V_S, \; \psi_S(u) = t_M $ (ii) $\forall x \in V_S, \; l(x) = l_M(\psi_S(x))$ and (iii)  $\forall x,y \in V_S, \; (x,y) \in E_S$ if $ (\psi_S(x), \psi_S(y)) \in E_M$.}

\textcolor{red}{The receptive field around a target $t_M$ is defined by the context $c_M$ and auxiliary nodes $B_M$ in motif $M$. Note that though $t_M$ is locally connected to just $c_M$ through motif $M$, we also include the auxiliary nodes $B_M$ in the receptive field since they provide useful 
features for convolution.}
%The set of all instances of $M$ in $G$ with target node $u$ denoted by $I^M_{u}$, constitute the region spanned by the receptive field (motif $M$) around target $u$.  %In homogeneous graphs, the receptive field defined by a motif is potentially applicable on all nodes.
The structural roles of various nodes w.r.t target $u$ in an instance $S_u \in I^M_{u}$  (the set of all instances of $M$ in $G$ with target $u$) can be easily deduced from the structure and types of nodes in $M$. %The number of unique structural roles in $M$ is given by $K_M (< |C_M|)$.
Thus, we denote $\phi(V_S, E_S, u, c)$, a role mapping function that takes an instance $S_u = (V_S, E_S)$, target $u \in V_S$, node $v \in V_S$ and returns the structural role ($\in \{ 1, \dotsc, K_M\}$) of $v$ relative to $u$.
